Local Search GFlowNets

Generative Flow Networks (GFlowNets) are amortized sampling methods that learn a distribution over discrete objects proportional to their rewards. GFlowNets exhibit a remarkable ability to generate diverse samples, yet occasionally struggle to consistently produce samples with high rewards due to over-exploration on wide sample space. This paper proposes to train GFlowNets with local search, which focuses on exploiting high-rewarded sample space to resolve this issue. Our main idea is to explore the local neighborhood via backtracking and reconstruction guided by backward and forward policies, respectively. This allows biasing the samples toward high-reward solutions, which is not possible for a typical GFlowNet solution generation scheme, which uses the forward policy to generate the solution from scratch. Extensive experiments demonstrate a remarkable performance improvement in several biochemical tasks. Source code is available: \url{https://github.com/dbsxodud-11/ls_gfn}.

==> tables/table2.tex <==
% \begin{table*}[h]
% \centering
% \caption{{Perfomance evaluation of 
%  average reward, diversity, and a unique fraction of the Top 128 samples.}}\label{tab:orignal_table}
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{llllllll}
% \toprule
%  Method&Type&\multicolumn{3}{c}{QM9}&\multicolumn{3}{c}{RNA ($L=14$)}
%  \\
%  &&Avg. Reward &Diversity&Uniq. Fraction &Avg. Reward &Diversity&Uniq. Fraction\\
% \midrule

% A2C
% &
% RL
% &

% &

% &

% &

% &

% &

% \\


% PPO
% &
% RL
% &

% &

% &

% &

% &

% &

% \\
% \midrule
% Back $\&$ Forth
% & 
% MCMC
% &

% &

% &

% &

% &

% &

% \\
% MARS
% &
% MCMC
% &

% &

% &

% &

% &

% &

% \\
% \midrule
% DB
% &
% GFN
% &

% &

% &

% &

% &

% &


% \\
% TB
% &
% GFN
% &
% 0.56 $\pm$ 0.01
% &
% \textbf{0.43 $\pm$ 0.00}
% &
% \textbf{0.99 $\pm$ 0.00}
% &
% 0.45 $\pm$ 0.01
% &
% 3.61 $\pm$ 0.04
% &
% 1.00 $\pm$ 0.00
% \\
% Sub-TB
% &
% GFN
% &

% &

% &

% &

% &

% &

% \\
% GTB
% &
% GFN
% &
% &

% &

% &

% &

% &

% \\
% MC-GFN (\textit{ours})
% &
% GFN
% &
% 0.57 $\pm$ 0.01
% &
% \textbf{0.43 $\pm$ 0.00}
% &
% 0.98 $\pm$ 0.00
% &
% \textbf{0.61 $\pm$ 0.01}
% &
% 3.02 $\pm$ 0.09
% &
% \textbf{1.00 $\pm$ 0.00}
% \\


% \bottomrule
% \end{tabular}
% }
% \vspace{-10pt}
% \end{table*}


% \begin{table*}[h]
% \centering
% \caption{{Perfomance evaluation on various metric on RNA generation task.}}\label{tab:orignal_table}
% \resizebox{0.85\linewidth}{!}{
% \begin{tabular}{llllllll}
% \toprule
%  Method&Type&Num. Modes & 100th per& 50th per &Diversity &Uniq. Fraction\\
% \midrule

% SQL
% &
% RL
% &



% &

% &

% &

% &

% \\


% PPO
% &
% RL
% &



% &

% &

% &

% &

% \\
% \midrule
% Back $\&$ Forth
% & 
% MCMC
% &

% &

% &

% &

% &

% &

% \\
% MARS$^\dagger$
% &
% MCMC
% &

% &

% &

% &

% &

% &

% \\
% \midrule
% DB
% &
% GFN
% &

% &

% &

% &

% &

% &


% \\
% TB
% &
% GFN
% &

% &

% &

% &

% &

% &
% \\
% MatEnt
% &
% GFN
% &

% &

% &

% &

% &

% &
% \\
% Sub-TB
% &
% GFN
% &

% &

% &

% &

% &

% &

% \\
% GTB
% &
% GFN
% &
% &

% &

% &

% &

% &

% \\
% MC-GFN (\textit{ours})
% &
% GFN
% &

% &

% &

% &

% &

% &

% \\


% \bottomrule
% \end{tabular}
% }
% \vspace{-10pt}
% \end{table*}

\begin{table*}[h]
\centering
\caption{{Perfomance evaluation of 
 the the number of discovered modes}}\label{tab:orignal_table}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lllllll}
\toprule
 Method&QM9&sEH&TFBind8 &RNA ($L=14$)&RNA ($L=50$)&RNA ($L=100$)\\
\midrule


DB

&

&

&

&

&

&


\\
TB

&

&

&

&

&

&
\\
MatEnt-TB

&

&

&

&

&

&
\\
Sub-TB

&

&

&

&

&

&

\\
GTB

&
&

&

&

&

&

\\
MC-GFN (\textit{ours})

&
\textbf{760} $\pm$ 4
&
000 $\pm$ 0
&
000 $\pm$ 0
&
28 $\pm$ 5
&
00 $\pm$ 0
&
00 $\pm$ 0
\\


\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}


==> tables/table3.tex <==
\begin{table*}[t!]
\centering
\caption{{Comparison with reward maximization methods on QM9 task.}}\label{tab:reward_maximization}
\resizebox{0.83\linewidth}{!}{
\begin{tabular}{llccl}
\toprule
 Method&Num. Modes &Top 100 Reward & Top 100 Diversity & Uniq. Fraction\\
\midrule
MARS
& 548 ± 22  & 0.65 ± 0.01 & \underline{0.41 ± 0.00} & 0.27 ± 0.01
\\
A2C - Entropy
& 344 ± 173 & 0.56 ± 0.04 & 0.38 ± 0.02 & 0.06 ± 0.04
\\
Soft Q-Learning
& 231 ± 6 & 0.56 ± 0.01 & \textbf{0.43 ± 0.00} & \textbf{0.92 ± 0.00} 
\\
PPO
& 567 ± 70  & 0.63 ± 0.01 & \underline{0.41 ± 0.01} & 0.65 ± 0.10
\\
\midrule
TB
& 699 ± 14  & 0.66 ± 0.00 & \underline{0.41 ± 0.00} & \underline{0.85 ± 0.00} 
\\
LS-GFN (\textit{Stochastic}) + TB
& \underline{771 ± 2} & \textbf{0.67 ± 0.00} & \underline{0.41 ± 0.00} & 0.76 ± 0.00
\\
LS-GFN (\textit{Deterministic}) + TB
& \textbf{793 ± 4}  & \textbf{0.67 ± 0.00} & \underline{0.41 ± 0.00} & 0.74 ± 0.00 
\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}

==> tables/table_append_2.tex <==
\begin{table*}[h!]
\centering
\caption{{RL Hyperparameter Search Space}}\label{tab:mlp_hyperparameters_rl}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
 Model & Learning rate & Entropy coefficient \\
\midrule
A2C & $\{1\times10^{-5}, \bm{1\times10^{-4}}, 1\times10^{-4}, 5\times10^{-3}, 1\times10^{-3}\}$ & $\{1\times10^{-4}, 1\times10^{-3}, \bm{1\times10^{-2}}\}$ \\
Soft Q-Learning & $\{1\times10^{-5}, \bm{1\times10^{-4}}, 1\times10^{-4}, 5\times10^{-3}, 1\times10^{-3}\}$ & - \\
PPO & $\{1\times10^{-5}, \bm{1\times10^{-4}}, 1\times10^{-4}, 5\times10^{-3}, 1\times10^{-3}\}$ & $\{1\times10^{-4}, 1\times10^{-3}, \bm{1\times10^{-2}}\}$ \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}
